Can Diffusion Model Achieve Better Performance in Text Generation? Bridging the Gap between Training and Inference!

Diffusion models have been successfully adapted to text generation tasks by mapping the discrete text into the continuous space. However, there exist nonnegligible gaps between training and inference, owing to the absence of the forward process during inference. Thus, the model only predicts based on the previously generated reverse noise rather than the noise computed by the forward process. Besides, the widely-used downsampling strategy in speeding up the inference will cause the mismatch of diffusion trajectories between training and inference. To understand and mitigate the above two types of training-inference discrepancies, we launch a thorough preliminary study. Based on our observations, we propose two simple yet effective methods to bridge the gaps mentioned above, named Distance Penalty and Adaptive Decay Sampling. Extensive experiments on \textbf{6} generation tasks confirm the superiority of our methods, which can achieve $100\times \rightarrow 200\times$ speedup with better performance.

==> table/case/case_studt_roc_bk.tex <==
\begin{table*}[t]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{c | l | l }
\toprule
Case & Type & Text \\
\midrule
\multirow{1}{*}{1} & Prompt & i was on my laptop computer. \\
    \cmidrule{2-3}
     & Origin (2000) & \makecell[l]{all of a sudden my computer stopped working on the table. i was scared because it ripped so i ended up buying it. \\ i went to the store to get a new one. after half of my computer, the screen were fine.} \\
     \cmidrule{2-3}
     & + Ours (2000) & \makecell[l]{all of a sudden my computer stopped working. the screen was broken. \\ it was so frustrated i had to get a replacement. luckily i was able to fix.} \\
     \cmidrule{2-3}
     & + Respace (20) & \makecell[l]{all of a sudden my computer \textcolor{blue}{stopped and stopped} working. i was very shocked and realized it was my computer. \\ i called to the coffee again and had to buy a new one. after paying the work, my new computer broke.}\\
     \cmidrule{2-3}
     & + Ours (20) & \makecell[l]{all of a sudden my computer stopped. it broke the screen. \\ it was not flying and i took it back to the store to fix it. luckily, it was fixed.}\\
\midrule
\multirow{1}{*}{2} & Prompt & alex has a big exam on friday. \\
    \cmidrule{2-3}
     & Origin (2000) & \makecell[l]{he has been studying all week. he got out of class. he got into class instead. his teacher gave the test and knew and made \\ an a.} \\
     \cmidrule{2-3}
     & + Ours (2000) & \makecell[l]{he has been studying all week. he got to class. when he got to class, his teacher handed out the test. alex was thrilled.} \\
     \cmidrule{2-3}
     & + Respace (20) &\makecell[l]{he has been studying all week. he got to class ready. he got into class. and his teacher got it. alex was chosen nervous  \\and a slept.} \\
     \cmidrule{2-3}
     & + Ours (20) &\makecell[l]{he has been studying all week. he stayed up all night. he got to class days early. alex took the test and was so happy!} \\
\midrule
\multirow{1}{*}{3} & Prompt & terry is driving home. \\
    \cmidrule{2-3}
     & Origin (2000) & \makecell[l]{he sees a dog in the road. he gets over to see what the dog is. he pulls it to be put out.} \\
     \cmidrule{2-3}
     & + Ours (2000) & \makecell[l]{terry sees a dog on the road. his car starts to get over. he see's coming. he is relieved and \textcolor{blue}{he calls by the calls} for help.}\\
     \cmidrule{2-3}
     & + Respace (20) & \makecell[l]{terry sees a dog in the road. he gets over to pull over it. it is all over. he got help and and out.} \\
     \cmidrule{2-3}
     & + Ours (20) & \makecell[l]{terry sees a dog in the road. he gets over to pull over it. it is all over. he got help and and out.} \\
\midrule
\multirow{1}{*}{4} & Prompt & kate lost her cat. \\
    \cmidrule{2-3}
     & Origin (2000) & \makecell[l]{she looked everywhere for it. she kept really up to make it. eventually they found it and found her cat. kate's cat stopped.} \\
     \cmidrule{2-3}
     & + Ours (2000) & \makecell[l]{she looked everywhere for it. eventually she gave for help. eventually she found it and looking for it. they got good at cat.}\\
     \cmidrule{2-3}
     & + Respace (20) & \makecell[l]{she looked everywhere for it. she kept not to friends about it. \textcolor{blue}{eventually she found it and finally found it}. kate found her cat.} \\
     \cmidrule{2-3}
     & + Ours (20) & \makecell[l]{she looked everywhere for it. \textcolor{blue}{eventually she gave up some and eventually.} eventually she looked up and found the cat. \\ kate's neighbor eventually the tree. } \\


\midrule
\multirow{1}{*}{5} & Prompt & jo went up to the rooftop to work on her tan. \\
    \cmidrule{2-3}
     & Origin (2000) & \makecell[l]{she went out and and \textcolor{blue}{felt most of the day}. the other thing she went in the front lot. the end of out, there was a puddle. jo \\ had to be down and had a great time.} \\
     \cmidrule{2-3}
     & + Ours (2000) & \makecell[l]{she went out and anda, it was a lot of fun. jo went out of the sun. \textcolor{blue}{when the woman she was an a off}. jo looked out her and \\ and had to get a nice and out.}\\
     \cmidrule{2-3}
     & + Respace (20) & \makecell[l]{she went out and \textcolor{blue}{got was on the menu}. while watching the over jo put the on the backer.  most of the tan and it was empty. \\ jo had to use the and and was more hours.} \\
     \cmidrule{2-3}
     & + Ours (20) & \makecell[l]{she went out and had a lot of it. by the end, she played a few hours. it was in the end and she did. jo went out to be a the \\ and short. } \\


\midrule
\multirow{1}{*}{6} & Prompt & matthew had just finished high school. to work on her tan. \\
    \cmidrule{2-3}
     & Origin (2000) & \makecell[l]{he decided he needed to go to college. after test about 18, matthew decided he was going to cook an written working as a \\ chef. matthew won an a scholarship.} \\
     \cmidrule{2-3}
     & + Ours (2000) & \makecell[l]{he decided \textcolor{blue}{he needed to college to college.} he was eating a nap. he decided that he would make the other way outside. he \\ decided to take it home.}\\
     \cmidrule{2-3}
     & + Respace (20) & \makecell[l]{he decided he \textcolor{blue}{needed a place to college}. he started a week. matthew decided he would make an school. he decided to bring \\ his  application until he was known.} \\
     \cmidrule{2-3}
     & + Ours (20) & \makecell[l]{he decided he needed a good job. he didn't know \textcolor{blue}{what to do the the}. he realized he was not it with his teacher. he decided \\ he would never get a good scholarship. } \\

     
\bottomrule
\end{tabular}}
\caption{Representative generated results of the ROC testing set, where \textcolor{blue}{blue color} denotes the serious grammatical errors.}
\label{tab:case_1}
\end{table*}

==> table/denoise_steps.tex <==
\begin{table*}[!tbp]
    \centering
    \small
    \begin{tabular}{ll|c c c c c c c c }
    \toprule
    \textbf{Task} & \textbf{Model}  & \textbf{Step$\dagger$} & \textbf{B-2$\uparrow$} & \textbf{R-2$\uparrow$} & \textbf{D-4$\uparrow$} & \textbf{BS$\uparrow$} & \textbf{$\Delta$ PPL$\downarrow$} & \textbf{Mavue$\uparrow$} & \textbf{Rep-2$\downarrow$}\\
    \midrule
    \multirow{16}{*}{\makecell[l]{Paraphrase}} 
    &  \multirow{4}{*}{CMLM} & 1 & & & & & & & \\
    & & 20 & & & & & & & \\
    & & 200 & & & & & & & \\
    & & 2000 & & & & & & & \\
    \cmidrule{2-10}      
    &  \multirow{4}{*}{SeqDiff} & 1 & & & & & & & \\
    & & 20 & & & & & & & \\
    & & 200 & & & & & & & \\
    & & 2000 & & & & & & & \\
    \cmidrule{2-10} 
    &  \multirow{4}{*}{+Respace} 
    &   2 & 0.2295 & 0.1371 & 0.4198 & & 0.5714 & 0.1216 & 0.0085 \\
    & & 5 & 0.3405 & 0.2084 & 0.5406 & & 0.7493 & 0.0294 & 0.2909 \\
    & & 20& 0.3874 & 0.2377 & 0.5926 & & 0.8223 & 0.0462 & 0.9123 \\
    & &200& 0.3941 & 0.2415 & 0.6026 & & 0.8425 & 0.0512 & 0.9466 \\
    \cmidrule{2-10} 
    &  \multirow{4}{*}{+Ours} 
    &   2 & 0.3386 & 0.2084 & 0.5233 & & 0.7326 & 0.0514 & 0.2285 \\
    & & 5 & 0.3998 & 0.2503 & 0.6002 & & 0.8285 & 0.0537 & 0.9335 \\
    & & 20& 0.4116 & 0.2579 & 0.6144 & & 0.8414 & 0.0519 & 0.9571 \\
    & &200& 0.4145 & 0.2588 & 0.6174 & & 0.8442 & 0.0565 & 0.9653 \\
    \bottomrule
    \end{tabular}
    \caption{Unconstrained text generation results. As for CMLM model, we report the iterative refinement steps and denoising steps for diffusion models.}
    \label{tab:main_tab}
\end{table*}
